MEV Capture and Decentralization in Execution Tickets

We provide an economic model of Execution Tickets and use it to study the ability of the Ethereum protocol to capture MEV from block construction. We demonstrate that Execution Tickets extract all MEV when all buyers are homogeneous, risk neutral and face no capital costs. We also show that MEV capture decreases with risk aversion and capital costs. Moreover, when buyers are heterogeneous, MEV capture can be especially low and a single dominant buyer can extract much of the MEV. This adverse effect can be partially mitigated by the presence of a Proposer Builder Separation (PBS) mechanism, which gives ET buyers access to a market of specialized builders, but in practice centralization vectors still persist. With PBS, ETs are concentrated among those with the highest ex-ante MEV extraction ability and lowest cost of capital. We show how it is possible that large investors that are not builders but have substantial advantage in capital cost can come to dominate the ET market.

==> conclusion.tex <==
This paper presents a comprehensive economic model of ETs and their potential to internalize MEV within the Ethereum blockchain. Our analysis reveals that ETs can fully internalize MEV under ideal conditions where builders are homogeneous, risk-neutral, and face no capital costs. However, the efficiency of MEV extraction diminishes significantly with increased risk aversion, capital costs, and builder heterogeneity. We explain that the current dominance of a few builders in the MEV-Boost system could persist or even intensify with the implementation of ETs.

We also highlight several limitations of the current model, including that it does not account for exogenous factors, the complexities of multi-block MEV, the intricacies of primary and secondary market dynamics for ETs, and the identification of actors involved in the process. Moreover, this paper does not compare ETs to other proposed MEV capture solutions, such as EAs.
